Auto-ICL: In-Context Learning without Human Supervision

With in-context learning ability, the performance of large language models can be significantly boosted when provided with appropriate context. However, existing in-context learning methods mainly rely on human-provided contexts, such as labeled examples and explicit instructions. Writing context by humans is labor-intensive on various tasks and limits the model to tasks manageable by humans. To overcome these limitations, we propose Automatic In-Context Learning framework that enables the model to autonomously generate examples and instructions for problem-solving. With experiments across various models and datasets, results show that model-generated contexts outperform human-annotated contexts, including Few-Shot and Few-Shot-CoT methods, and surpass existing self-generated context methods like Zero-CoT and Auto-CoT.

==> templates/test.tex <==
\begin{longtable}{@{}l| p{2.5cm}| p{2.5cm}@{}}
\hline
\textbf{Dataset} & \textbf{Question} & \textbf{Instruction}\\
\hline
TOMI1 & Ava entered the sunroom. Lily entered the sunroom. Ava loves the skirt. The asparagus is in the bathtub. Ava exited the sunroom. Lily moved the asparagus to the pantry. Lily dislikes the skirt. Lily exited the sunroom. Ava entered the garage. Where will Ava look for the asparagus? Answer Choices: (A) bathtub (B) pantry (C) Unknown & 1. Read the given information carefully to understand the sequence of events.
2. Identify the key details in the passage, such as the location of the asparagus and the actions of Ava and Lily.
3. Note that Ava entered the sunroom and Lily moved the asparagus to the pantry after Ava left.
4. Since Ava did not witness Lily moving the asparagus, she would not know that it was moved to the pantry.
5. Therefore, Ava would most likely look for the asparagus in its original location, which is the bathtub.
6. Therefore, the answer is (A) bathtub. \\
\hline
TOMI2 & Mason entered the laundry. Alexander dislikes the underpants. Alexander entered the laundry. The onion is in the treasure chest. Mason exited the laundry. Alexander moved the onion to the crate. Ella likes the pajamas. Alexander exited the laundry. Mason entered the laundry. Where does Mason think that Alexander searches for the onion? Answer Choices: (A) Unknown (B) treasure chest (C) crate
&  1. Read the given information carefully to understand the sequence of events.
2. Identify the key characters and objects mentioned in the question.
3. Note down the actions performed by each character and the location of the objects.
4. Analyze the information to determine where Mason thinks Alexander searches for the onion.
5. Eliminate answer choices that are not supported by the given information.
6. Choose the answer choice that is the most logical based on the given information.
7. Verify the answer by checking if it aligns with the sequence of events and actions performed by the characters. \\
\hline
SocialIQA & Riley is the most popular student in the school. What will Others want to do next? Answer Choices: (A) run for class president (B) run for student council (C) join Riley's gang
& 1. Identify the reasons why Riley is the most popular student in the school.
2. Analyze the characteristics of Riley's popularity and determine what aspects of it others may want to emulate.
3. Consider the potential motivations of the other students and what they hope to achieve by following in Riley's footsteps.
4. Evaluate the answer choices provided and determine which option aligns best with the motivations and goals of the other students.
5. Choose the answer choice that best fits the situation. \\
\hline
Coin Flip &  A coin is heads up. Bill flips the coin. Santos does not flip the coin. Roxy flips the coin. Randi flips the coin. Is the coin still heads up? Note that "flip" here means "reverse". & 1. Determine the starting position of the coin (heads up).
2. Understand the meaning of "flip" in this context (reverse).
3. Determine the order of the flips: Bill, Santos, Roxy, Randi.
4. Apply the flip to the starting position of the coin for each person in the order given.
5. Determine the final position of the coin after all flips have been applied.
6. Compare the final position to the starting position to determine if the coin is still heads up. \\
\hline
Last Letter& Take the last letters of each words in "Rena Devon Rosalinda Paulina" and concatenate them. & 1. Identify the given words: "Rena Devon Rosalinda Paulina"
2. Determine the last letter of each word.
3. Write down the last letters of each word.
4. Concatenate the last letters in the order they appear in the original phrase.
5. Verify that the resulting string is correct. \\
\hline
MultiArith & Paige and her friends were recycling paper for their class. For every 4 pounds they recycled they earned one point. If Paige recycled 14 pounds and her friends recycled 2 pounds, how many points did they earn? & 1. Determine the total weight of paper recycled by Paige and her friends. 
2. Add the weight of paper recycled by Paige and her friends. 
3. Divide the total weight of paper recycled by 4 to determine the number of points earned. 
4. Round the answer to the nearest whole number, as points are given in whole numbers. 
5. Write the final answer in the form of a sentence. \\
\hline
AQUA & In a row of children Neha is 12th from left end and Radha is 6th from right end. When Radha is shifted to left by 2 places and Neha is shifted to right by 2 places there 6 children between Radha and Neha. How many children are there in the row? Answer Choices: (A) 23 (B) 27 (C) 26 (D) 28 (E) 29 & 1. Draw a diagram to represent the given information.
2. Use the information given to determine the total number of children in the row.
3. Determine the original positions of Neha and Radha in the row.
4. Determine the new positions of Neha and Radha after they are shifted.
5. Use the information given to determine the number of children between Neha and Radha after they are shifted.
6. Use the information gathered to solve for the total number of children in the row.
7. Check the answer choices and select the correct answer. \\
\hline
GSM8K&  Carly is making cupcakes and brownies for her art class. She makes 2 less than three times as many brownies as cupcakes. If Carly's class has five people and each person gets two treats, how many cupcakes did Carly make? & 1. Use algebra to set up an equation to represent the relationship between the number of cupcakes and brownies Carly made.
2. Solve the equation to find the number of brownies Carly made.
3. Use the number of brownies to find the number of cupcakes Carly made.
4. Multiply the number of cupcakes by 2 to find the total number of treats.
5. Divide the total number of treats by 10 (5 people x 2 treats per person) to find the number of cupcakes each person gets. \\
\hline
Cycle Letter & Please unscramble the letters into a word, and write that word: 
ebukkak = & 1. Identify the letters in the scrambled word: ebukkak.
2. Rearrange the letters to form a word.
3. Check if the word makes sense and is spelled correctly.
4. Write the unscrambled word. \\
\hline
Shuffle Object& Alice, Bob, and Claire are dancers at a square dance. At the start of a song, they each have a partner: Alice is dancing with Sam, Bob is dancing with Helga, and Claire is dancing with Karl. 

Throughout the song, the dancers often trade partners. First, Claire and Alice switch partners. Then, Bob and Alice switch partners. Finally, Claire and Bob switch partners. At the end of the dance, Alice is dancing with 
Which choice is true ? Answer Choices: (A) Sam. (B) Helga. (C) Karl. & 1. Understand the problem: Read the problem carefully and make sure you understand the given information and what is being asked.
2. Visualize the problem: Draw a diagram or use a table to keep track of the dancers and their partners before and after each switch.
3. Follow the steps: Follow the given steps in the problem and make sure to update the diagram or table after each switch.
4. Determine the final partner: After the final switch, determine who Alice is dancing with and compare it to the answer choices given.
5. Choose the correct answer: Select the answer choice that matches the final partner Alice is dancing with. \\
\hline
\end{longtable}




